Large area monocrystalline and surfactant-free copper microflake synthesis

Copper is one of the most extensively studied materials for energy conversion and catalytic systems, with a wide range of other applications from nanophotonics to biotechnology. However, existing synthesis methods are limited with many undesirable by-products and poorly defined morphologies. Here, we report a surfactant-free on-substrate wet synthesis approach that yields monocrystalline metallic Cu microflakes with (111) crystalline exposed surface. By systematically studying the growth mechanism, we achieve unprecedented sizes of more than 130 {\mu}m, which is two orders of magnitude larger than reported in most previous studies, along with higher aspect ratios of over 400. Furthermore, we show distinctly higher stability against oxidation provided by the halide adlayer. Overall, our facile synthesis approach delivers an exciting venue for the emerging fields of catalysis and nanophotonics.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
\newcommand{\RomanNumeralCaps}[1]
    {\MakeUppercase{\romannumeral #1}}
   % \usepackage[utf8]{inputenc}
%\DeclareUnicodeCharacter{200B}{}
\usepackage[utf8]{inputenc} % For UTF-8 support (for older versions of LaTeX)
\usepackage{newunicodechar}
\newunicodechar{​}{}
\DeclareUnicodeCharacter{2009}{\,}

